ArtInsight: Enabling AI-Powered Artwork Engagement for Mixed Visual-Ability Families

We introduce ArtInsight, a novel AI-powered system to facilitate deeper engagement with child-created artwork in mixed visual-ability families. ArtInsight leverages large language models (LLMs) to craft a respectful and thorough initial description of a child's artwork, and provides: creative AI-generated descriptions for a vivid overview, audio recording to capture the child's own description of their artwork, and a set of AI-generated questions to facilitate discussion between blind or low-vision (BLV) family members and their children. Alongside ArtInsight, we also contribute a new rubric to score AI-generated descriptions of child-created artwork and an assessment of state-of-the-art LLMs. We evaluated ArtInsight with five groups of BLV family members and their children, and as a case study with one BLV child therapist. Our findings highlight a preference for ArtInsight's longer, artistically-tailored descriptions over those generated by existing BLV AI tools. Participants highlighted the creative description and audio recording components as most beneficial, with the former helping ``bring a picture to life'' and the latter centering the child's narrative to generate context-aware AI responses. Our findings reveal different ways that AI can be used to support art engagement, including before, during, and after interaction with the child artist, as well as expectations that BLV adults and their sighted children have about AI-powered tools.

==> ModelComparisonTables.tex <==
\newcommand{\firsttable}{
\begin{table*}[h]
  \centering
  \renewcommand{\arraystretch}{1.2}
  \resizebox{\textwidth}{!}
  {
    \begin{tabular}{p{0.07\linewidth} p{0.31\linewidth} p{0.31\linewidth} p{0.31\linewidth}} % Adjust column widths as needed
      \textbf{}
       & \begin{minipage}{.25\textwidth}
          \includegraphics[width=\linewidth]{raw_art/rainbow.png}
          \textbf{\textit{Rainbow}}
          \Description{A child's artwork of a rainbow with seven colors, a pot of gold on the bottom right of the rainbow, a green grassy ground, a blue sky, and a yellow sun at the top right of the artwork.}
        \end{minipage} 
        & \begin{minipage}{.25\textwidth}
          \includegraphics[width=\linewidth]{raw_art/abstract_blue_white_red.png}
          \textbf{\textit{AbstractBlueWhiteRed}}
          \Description{An abstract artwork with a dark blue background, some white paintbrush strokes in a circular shape, and a red ghost-like figure in the center-right that has been done on a cut-out piece of paper on top of the blue background paper.}
          \end{minipage} 
        & \begin{minipage}{.2\textwidth}
          \includegraphics[width=\linewidth]{raw_art/peeps.png}
          \textbf{\textit{Peeps}}
          \Description{A coloring book page with several "Peeps" outlined in black, and a few peeps colored in throughout the page in various shades of red, green, yellow, blue, and purple. The bottom right of the page has some words that read: "Express your Peepsonality".}
          \end{minipage} 
        \\
      \hline
        \textbf{Claude 3.5 Sonnet}
        &
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          3 & 4 & 4 & 4 \\
          \hline
        \end{tabular}
        % \vspace{0.2em}
        \newline
        Makes assumptions, such as the black object being a "pot or cauldron" and the yellow line representing "gold or something valuable inside."
        & 
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          2 & 4 & 4 & 4 \\
          \hline
        \end{tabular}
        % \vspace{0.2em}
        \newline
        Assumptions include the red figure being a "person or creature" and suggesting themes like "isolation, adventure, or standing out in a chaotic world." 
        &
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          2 & 4 & 4 & 3 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Assumes blue shape may be a "gingerbread man or a little person." Assumes purpose of the text. Should specify the placement of colors. \hfill

        \textit{-1 Misc}: Misidentifies the blue shape.
        \\
        \hline
        \textbf{Score}
        &
        \textbf{15/16}
        & 
        \textbf{14/16}
        &
        \textbf{12/16}
        \\
        \hline
        \textbf{GPT-4 Turbo}
        &
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          3 & 4 & 4 & 4 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Makes an assumption about child intent: the black pot with a yellow band is "the classic tale of a pot of gold at the end of the rainbow."
        & 
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          2 & 4 & 4 & 4 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Assumptions about the intent and themes: "a moment of calm... within a stormy or chaotic environment," and "themes such as peace amid chaos..."
        &
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          3 & 4 & 4 & 4 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Assumes intent, such as: the choice to color one Peep differently is due to "a sense of standing out" and "mirroring a personal expression."
        \\
        \hline
        \textbf{Score}
        &
        \textbf{15/16}
        & 
        \textbf{14/16}
        &
        \textbf{15/16}
        \\
        \hline
        \textbf{GPT-4o}
        &
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          4 & 4 & 4 & 4 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Respectful and celebrates the child's creativity with positive language like "joyful" and "vibrant", is detailed and covers colors and brushstrokes, and captures all major elements.
        & 
       \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          2 & 4 & 4 & 4 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Suggesting the background is a "night sky or deep space" and that the red figure "might be a character wearing a hood or a cloak." \hfill

        \textit{-1 Misc}: Asking "What does your child say about their creation?"
        &
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          4 & 4 & 4 & 4 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Avoids making assumptions, is respectful and uses positive language like "fun and eye-catching pattern", is detailed and covers aspects like colors and placement, and captures all major elements.
        \\
        \hline
        \textbf{Score}
        &
        \textbf{16/16}
        & 
        \textbf{13/16}
        &
        \textbf{16/16}
        \\
        \hline
        \textbf{Gemini 1.5 Flash}
        &
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          2 & 4 & 3 & 4 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Too simple, makes assumptions about the intent behind the artwork ("fun day"), asks speculative questions. \hfill

        \textit{-1 Misc}: Asking "What do you think it represents to your child?".
        & 
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          1 & 3 & 2 & 3 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Assumptions about the white areas "look like clouds", the scene is "in the sky". Saying "maybe this is a scene in the sky?" could be minimizing to the child's effort. Also too simple and not all major elements captured. \hfill

        \textit{-1 Misc}: Asks "What do you think?"
        &
        \begin{tabular}{| p{0.17\linewidth} | p{0.16\linewidth} | p{0.17\linewidth} | p{0.17\linewidth} |}
          \textbf{R.A} & \textbf{R.B} & \textbf{R.C} & \textbf{R.D} \\
          \hline
          4 & 4 & 3 & 3 \\
          \hline
        \end{tabular}
        %\vspace{0.2em}
        \newline
        Could provide more detail about the specific arrangement and the overall pattern of the figures. Also misses identifying the text, "Express your Peepsonality".
        \\
        \hline
        \textbf{Score}
        &
        \textbf{12/16}
        & 
        \textbf{8/16}
        &
        \textbf{14/16}
        \\
        \hline
    \end{tabular}
  }
  %\vspace{0.4em}
  \caption{Three example images from our dataset with the LLM Scorer scores for each Rubric guideline (R.A---presumptive, R.B---reductive, R.C---too simple, R.D---all elements captured), the reasoning for points lost, and the total scores.}
  \label{MasterTable}
\end{table*}
}

